Fuzzing+Hardware Performance Counters-Based Detection of Algorithm Subversion Attacks on Post-Quantum Signature Schemes

NIST is standardizing Post Quantum Cryptography (PQC) algorithms that are resilient to the computational capability of quantum computers. Past works show malicious subversion with cryptographic software (algorithm subversion attacks) that weaken the implementations. We show that PQC digital signature codes can be subverted in line with previously reported flawed implementations that generate verifiable, but less-secure signatures, demonstrating the risk of such attacks. Since, all processors have built-in Hardware Performance Counters (HPCs), there exists a body of work proposing a low-cost Machine Learning (ML)-based integrity checking of software using HPC fingerprints. However, such HPC-based approaches may not detect subversion of PQC codes. A miniscule percentage of qualitative inputs when applied to the PQC codes improve this accuracy to 98%. We propose grey-box fuzzing as a pre-processing step to obtain inputs to aid the HPC-based method.

==> 02_threats.tex <==
\section{Threat Model}
\label{sec:threat}
Our threat model is in line with the setting proposed in \cite{threatModel}. We have four players in the setting: \textit{Saboteur}, \textit{Victim}, \textit{Attacker}, and \textit{Defender}. The goal of the \textit{Saboteur} is to stealthily weaken the PQC software, which may later be exploited by an \textit{Attacker} to target specific user(s) and recover their  secret keys or sensitive information. The \textit{victim} is the user who deploys the weakened PQC software. The \textit{defender} is the algorithm-level designer of the PQC software. The goal of the \textit{Defender} is to ensure that \textit{Victim} can easily check the integrity of the PQC software implementations. We encourage the reader to go through \cite{threatModel} for more details. We motivate our threat model using the classic FREAK~\cite{freak} attack, where the \textit{Saboteur} was allegedly the National Security Agency (NSA). They intentionally weakened the OpenSSL protocols by restricting to use RSA\_export key size below 512 bits. This can be easily decrypted by number field sieve factorization algorithm  using modest computing resources. NIST in its role of a \textit{Defender} has to ensure that the \textit{victim} can check for weaknesses in implementations. We assume PQC implementations in TLS/SSL libraries can be subverted intentionally or accidentally by software developers.
